Neutron Star Mergers and How to Study Them

Neutron star mergers are the canonical multimessenger events: they have been observed through photons for half a century, gravitational waves since 2017, and are likely to be sources of neutrinos and cosmic rays. Studies of these events enable unique insights into astrophysics, particles in the ultrarelativistic regime, the heavy element enrichment history through cosmic time, cosmology, dense matter, and fundamental physics. Uncovering this science requires vast observational resources, unparalleled coordination, and advancements in theory and simulation, which are constrained by our current understanding of nuclear, atomic, and astroparticle physics. This review begins with a summary of our current knowledge of these events, the expected observational signatures, and estimated detection rates for the next decade. I then present the key observations necessary to advance our understanding of these sources, followed by the broad science this enables. I close with a discussion on the necessary future capabilities to fully utilize these enigmatic sources to understand our universe.

==> bib_notes.tex <==
\citep{GW170817-MMAD} 
Multi-messenger Observations of a Binary Neutron Star Merger

Great overview of the history, with citations
Citations to all the initial science for 170817 (linear polarimetry show no evidence for asymmetric geometry - Covino)


\citep{GW170817-GW}
GW170817: Observation of Gravitational Waves from a Binary Neutron Star Inspiral

GW network: 3 'Fabry-Perot-Michelson interferometers'
insight into 'astrophysics, dense matter, gravitation, and cosmology'
GW SNR 18.8, 26.4, 2.0; set to GBM horizon distance for comparison


==> old_text.tex <==















\section{An Overview of Neutron Star Mergers}
\label{sec:NS_mergers_overview}

\ac{NS} mergers may produce all four of the astrophysical messengers across wide ranges in energies and time, as shown in Figure \ref{fig:observing_windows}. There are three canonical signals of \ac{NS} mergers: a chirping \ac{GW}, \acp{SGRB}, and kilonova. We first focus on a phenomenological description of these three signatures followed by a discussion on other possible observables. We do not here give an overview of the history of these topics, as we are unlikely to exceed existing literature; for a general history of our understanding of these sources we refer the reader to the introduction of \citet{GW170817-MMAD}.




\subsection{Gravitational Waves from Neutron Star Mergers}
\label{sec:GWs_from_NS}

\textcolor{blue}{somewhere discuss tidal effects on inspiral, and degeneracy breaking}

The earliest signal announcing a \ac{NS} merger will come in the form of \acp{GW}. The current accepted theory of gravity is Einstein's \ac{GR} \citep{einstein_GR_1916}, which he used to predict the existence of \acp{GW} \citep{einstein_GWs_1918}. This was the second to last of Einstein's predictions to be directly proven observationally, and it took a century \citep{GW150914}. While we expect to detect \acp{GW} from many sources in the future, the final inspiral and merger of compact objects (\acp{NS} and \acp{BH}) are the canonical \ac{GW} signals for ground-based interferometers because they are relatively short, have theoretically predicted waveforms used in sensitive template matching searches, and are loud and common enough to be regularly detected. The \ac{GW} signal is known to chirp, making it relatively distinct from most background contamination.

The current active \ac{GW} detectors are GEO600 \citep{GEO_600_Dooley_2016}, Advanced LIGO \citep{AdvLIGO}, and Advanced Virgo \citep{AdvVirgo}. GEO600 is a testbed of new technologies to improve the other detectors and is significantly less sensitive in the lower frequencies (where most \ac{GW} SNR is accumulated). These interferometers are expected to be joined by KAGRA \citep{KAGRA} in the next few years, and LIGO-India \citep{LIGO_India} a few years later. We refer to this network as the Gen 2 \ac{GW} network, and an overview of the expected sensitivity, localization capability, and rates is available in \citet{Gen_2_Prospects_2018}. 

There are several proposed future \ac{GW} detectors. The A+ upgrade of Advanced LIGO \textcolor{orange}{G1601435-v3 ? } has now been approved by the National Science Foundation (NSF), which could be implemented by 2024. The upgrade to the maximal sensitivity achievable within the existing LIGO interferometer arms is LIGO Voyager \textcolor{orange}{citation?}. We refer to these, and other upgrades of existing interferometers, as Gen 2.5 instruments. Grander proposals exist to build interferometers with arms several times longer than those that currently exist \citep{Einstein_Telescope, Cosmic_Explorer} with vast sensitivity increases that could detect \ac{BNS} mergers to a redshift of a few. We refer to these as Gen 3. Since these are all expected future sensitivities we list our assumptions in Appendix \ref{sec:GW_detection_rates} This includes nominal sensitivities, rates, and localization capabilities. Our expected scientific results are not particularly sensitive to the achieved sensitivity for a given generation. 

For \ac{BNS} mergers, coalescence may result in a prompt collapse to a \ac{BH}, a short-lived ($\sim<$1 s) \ac{HMNS} which is supported against collapse by differential rotation, a longer-lived \ac{SMNS} which is supported against collapse by uniform rotation, or a stable \ac{NS}. \ac{EM} observations can favor one outcome over the others, but there is likely to be ambiguity (see the on-going debate on the final remnant of \gwid \textcolor{orange}{bunch of citations}); however, \ac{GW} interferometers with sufficient high frequency ($\sim$kHz) sensitivity could directly measure coalescence and delineate between outcomes \textcolor{orange}{citation}. These firm observations could be used to understand the specific \ac{EM} signatures for each outcome. \ac{NSBH} mergers only result in a \ac{BH} since one already exists.

In addition to the ground-based interferometers, there are proposal for space-based interferometers that allow for arm lengths of millions of kilometers. \ac{LISA} has been accepted for launch by the European Space Agency with some NASA contribution. It nominally launches in 2034 and will be sensitive in the $\sim$mHz range (compared to the $\sim$kHz range for ground-based interferometers). Therefore, it will be sensitive to \ac{BNS} mergers from years to millions of years before merger, and \ac{NSBH} mergers from about a year to hundreds of millennia before merger; however, \textcolor{cyan}{given the rates of these systems we do not expect to detect any \ac{NS} merger near the end of their inspirals with \ac{LISA}}. Both the Gen 3 ground-based interferometers and \ac{LISA} approach the 1 Hz regime, but are not sensitive in this range. There are proposed space-based missions with shorter arm lengths (relative to \ac{LISA}) such as DECIGO, the Big Bang Observatory (BBO), MAGIS \textcolor{orange}{,etc and citations}. Such an instrument would be ideal for early warning systems with reasonable localizations, but they are at least decades away from launch. Lastly, there are \ac{GW} detectors in the nHz range that use sensitive timing observations of pulsars as effective interferometer arms, but even if a \ac{NS} system could be detected by these instruments (which is \textcolor{cyan}{unlikely because they would become unbound, and these detectors search for the mergers of the most massive black hole binaries)} they would not merge within millions of Hubble times.

\textcolor{cyan}{Tito it would be good to have a plot here showing the frequency evolution and time to merger with LISA and LIGO sensitivities. Maybe add assumed future ground-based sensitivities and DECIGO BBO MAGIS. Something like the Sesana plot?} \textcolor{red}{make this an appendix? - Appendix on GW instruments etc}



\subsection{Short Gamma-Ray Bursts}
\label{sec:SGRBs}

\acp{GRB} are the most luminous events in the Universe. Some brighter at Earth in gamma-rays than the rest of the Universe combined. They are cosmological transients with almost unparalleled energy scales. For two decades we have known that \acp{GRB} come in two classes: a short-hard class called \acp{SGRB} and a long-soft class called \acp{LGRB} \citep{Dezalay1991,Kouveliotou1993}. Based on a great deal of circumstantial evidence (see the reviews by \citealt{reviews_SGRBs_2007} or \citealt{review_SGRBs_Berger_2014}, or a compilation of follow-up observations in \citealt{fong2015decade} for details) it has long been believed that \ac{NS} mergers are the progenitors of \acp{SGRB} \citep{SGRB_progenitor_blinnikov_1984,SGRB_progenitor_NS_Goodman_1986,Paczynski1986,SGRBs_merging_NS_Eichler_1989} \textcolor{orange}{just cite a bunch of papers here}. \ac{BNS} mergers are now known to be a progenitor of \acp{SGRB} because of \gwid and \grbid \citep{GW170817-GRB170817A}. The confirmation that some \acp{SGRB} arise from \ac{NSBH} mergers, the relative fraction of each, and ruling out other possible progenitors are all key science drivers for future \ac{GW}-\ac{GRB} science.


\acp{GRB} are named because they were first identified as bursts of gamma-rays. This is the prompt phase of \acp{GRB} which is known to occur from keV to GeV energies (in some cases) and may extend far beyond this range. Based on theoretical arguments (e.g. the compactness problem) and observations of the afterglow it is believed that \acp{GRB} are emitted from ultrarelativistic jets \textcolor{orange}{cite Rhoads, Fong15, and specific jet breaks}. The leading emission mechanism is internal shocks caused by variable activity from the central engine, but this is not universally accepted (see Section \textcolor{blue}{sec ref}). Afterglow emission arises from synchrotron radiation when the bulk outflow interacts with the circumburst density. It is most prominent in X-rays (especially for \acp{SGRB}), has been observed from GeV through radio, and may extend to higher or lower energies.

The most prolific detector of \acp{SGRB} is the \Fermi \ac{GBM}. \ac{GBM} triggers on-board to about 50 \acp{SGRB}/year (here we use a $T_{90}$ division of 5 seconds, which is a more appropriate 50-50 boundary), which is more than every other active \ac{SGRB} detector combined. It further detects 100 \ac{SGRB} candidates through a blind sub-threshold search, and can search to even lower thresholds with a Targeted Search if given a seed time (and an optional location) \citep{Blackburn2015,Goldstein2016,Targeted_Search_Kocevski_2018}. The \Swift \ac{BAT} is unique among active \acp{GRB} detectors as it, along with its follow-up instruments \ac{XRT} and \ac{UVOT} \textcolor{orange}{cites}, provide arcsecond localizations to the follow-up community. This compares to \ac{GBM} \ac{SGRB} localization errors of $\sim$10 deg. There are several future proposed missions to detect \acp{SGRB} that range from CubeSats to probe-class missions. While \ac{NS} inspirals are standard sirens, the intrinsic luminosity distribution of \acp{SGRB} spans six orders of magnitude. This enables all-sky monitors to detect the brightest events to the edge of the visible universe.



\subsection{Kilonovae}
\label{sec:kilonova}

Shortly before merger the compact objects are moving at $\sim$0.5 c, which provides sufficient force to rend matter from \acp{NS}. \textcolor{blue}{More matter may be emitted at the shock front between \acp{NS} (in \ac{BNS} mergers) or from disk winds}. Bound material falls back and could power the \ac{SGRB}. Unbound ejecta is exceptionally neutron rich and undergoes rapid neutron capture (r-process), producing elements through lanthanides and actinides \textcolor{orange}{cite} \textcolor{blue}{Within a second}. This material, a few hundredths of a solar mass, expands outwards at a few tenths of the speed of light. As it expands, the neutron-heavy isotopes radioactively decay into more stable isotopes over the next few weeks. The material is optically thick at early times, allowing only neutrinos to escape. Next are gamma-rays on the \textcolor{blue}{hours} timescale \citep{kilonova_gamma_rays_hotokezaka_2016}. Neither of these signatures are detectable by any current mission. Kilonova have been divided into blue and red versions. Blue kilonova can occur when the material is relatively neutron-poor and therefore relatively lanthanide-free. This results in lower opacities and the escape of photons when the thermal emission peaks in the blue range. Red kilonova are neutron rich and lanthanide rich, which have much higher opacities and do not allow photon escape until the temperature cools into the red or infrared range. 

With \knid we observed both a blue and a red kilonova. The blue kilonova is thought to arise from the polar region where higher velocities and lower neutron fraction \textcolor{blue}{higher electron fraction} prevent the production of large amounts of heavy elements. The red kilonova arose from the dynamical eject in the orbital plane. This is the only unambiguous kilonova, but a few others have been claimed. From the last decade of follow-up observations of \acp{SGRB} we can infer that kilonova have at least an order of magnitude variation in brightness \textcolor{orange}{cite}, based on the claimed kilonova being brighter than \knid (and some showing only red emission), and extremely constraining limits on relatively nearby \acp{SGRB}. 

Because there are so many facilities in the optical and infrared that range from wide-field discovery instruments to narrow follow-up instruments we do not attempt to discuss them all in detail. The \ac{UV} range is currently covered by HST, \Swift \ac{UVOT}, and \textcolor{orange}{that one ground-based UV claim}. Many facilities had to stop observing \knid before the emission faded below detection threshold due to Sun-constraints. However, the Earth-\textcolor{blue}{trailing} Spitzer saw the event in infrared at 74 days after merger \citep{gw170817_spitzer}. \textcolor{blue}{One may also expect \ac{UV} emission after about an hour caused by a neutron front \citep{KN_macronova_Kulkarni_2005}, which was the mechanism dubbed a macronova. We find it likely that kilonova will be used to refer to these events, regardless of the strict method of heating.}



\subsection{Other Neutron Star Merger Signatures}
\label{sec:signatures_other}

While these are the three canonical signatures, they are far from the only observational signals from \ac{NS} mergers. We expect these events to produce neutrinos and possibly cosmic rays. There are expectations for precursor signals, modifications to the canonical ones such as cocoon emission from an off-axis or failed jet, generic omnidirectional radio emission, and \textcolor{blue}{possible very late-stage emission}.


\subsubsection{Neutrinos}
\label{sec:signatures_neutrinos}

Because of their incredibly tiny (but non-zero mass) neutrinos interact with matter only rarely. Therefore, following the \ac{GW} emission the next detectable signal from \ac{BNS} mergers may be neutrinos. As the \acp{NS} disrupt and coalesce they may not undergo prompt collapse to a \ac{BH}. If this occurs the resulting \ac{NS} will be incredibly hot, at $\sim$20 MeV, a warmth neither \ac{NS} has felt since their births. Unfortunately, they are unlikely to enjoy the experience for long if they are supported against collapse by differential rotation, referred to as a a \ac{HMNS}, as they are likely to collapse to a \ac{BH} $\sim<$1 s. These transient \ac{NS} are about as luminous in MeV neutrinos as core-collapse supernova \textcolor{red}{cite Metzger, Fernandez, and...what was the other?}. 

For a long time \acp{GRB} were thought to be candidates for astrophysical sources of neutrinos. If the jets are hadronic in nature then by the photopion process \textcolor{red}{$\sim$MeV gamma-rays correspond to $\sim$TeV neutrinos}. Unfortunately, the ultrarelativistic behavior actually lessens the production of neutrinos by time dilation of the lifetimes of protons. While the prompt \ac{GRB} emission may produce neutrinos, extended emission or cocoon emission are now thought to be more promising sources. \textcolor{red}{TeV} neutrinos are expected $\sim$1 s to $\sim$100 s after merger time. \textcolor{red}{cite Kimura and Murase}.

Lastly, \textcolor{red}{if the remnant object is a stable \ac{NS} or a \ac{SMNS} (supported against collapse by uniform rotation) then we may expect EeV neutrinos on the order of $\sim$days to $\sim$months - cite Fang, Metzger}.

Indeed searches for all of these types of neutrinos were performed around \gwid by the ANTARES, IceCube, and Pierre Auger Observatory teams...\textcolor{red}{discuss paper} but no positive detections resulted. However, we note the MeV and EeV neutrino production is not expected for \ac{NSBH} mergers.


\subsubsection{Cosmic Rays}
\label{sec:signatures_CRs}

Much like the source of astrophysical neutrinos is unknown and it was once thought that maybe \acp{GRB} were the dominant source class, this is also true for \ac{UHECR}. And much like the neutrino case we now believe this is not true. If jets are hadronic and produce neutrinos, then they are also sources of \ac{UHECR}. Therefore, \ac{NS} mergers may also be sources cosmic rays. \textcolor{red}{There is also a paper on late-time production of CRs? Maybe in the stage analogous to SNR? Nebular? Match timescales to figure 1.}



\subsubsection{Cocoon Emission}
\label{sec:signatures_cocoon}

The gamma-ray detection was several orders of magnitude fainted than previously known events (while in general surprising, this was not entirely unexpected \textcolor{orange}{cite my Swift-GBM paper}), and the afterglow was absent until several days later, and is still being observed to date. This has caused a great deal of disagreement into the origin of this emission, with groups split between a choked \ac{GRB} (which doesn't explain the gamma-rays), cocoon emission (with the gamma-rays coming from shock breakout), or a structured but otherwise typical \ac{SGRB} jet that is off-axis. While on-going afterglow observations may be able to delineate between models (based on the shape of the curvature of the turnover, which began $\sim$6 months after merger) for \grbid, future observations can also prove decisive. Prompt \ac{GRB} behavior could tell the difference between models based on spectral analysis ($E_{peak}$, or time-resolved behavior) or the structure/variability of the \ac{GRB} (where fast variation is difficult to explain with cocoon emission). It is also likely that we missed the afterglow in the first few hours after event time due to a lack of observations. Because there were prompt gamma-rays, their likely had to be an immediate afterglow that faded below detection threshold before observations were made. Future prompt observations will allow us to distinguish between models by measurement the change of the afterglow over time.

\subsubsection{Precursors}
\label{sec:signatures_precursors}

\subsubsection{Late-Time Radio}
\label{sec:signatures_radio}

There are also expectations that radio observations may provide the most signals following \ac{NS} mergers. The general idea is the relativistic outflows (either the ultrarelativistic jet or the semi-relativistic kilonova) interacts with the surrounding media, \textcolor{red}{emitting synchrotron radiation for months to years after merger time \citep{omni_radio_KN_Piran_2012,omni_radio_general_Hotokezaka_2015,omni_radio_optimization_Hotokezaka_2016}. This will provide unique insights into \ac{NS} mergers, but because of the large \ac{GW} localizations and the large time offset between merger and radio signal it is difficult to prove a detected radio signal was associated with a given \ac{NS} merger without some intermediate localization information from some other source. This may be possible for particularly well localized \ac{GW} events and with the measurement of a redshift of an expected host galaxy for the radio-localized source, but it is not a general thing.}

\subsubsection{Nebular and Diffuse Emission(?)}
\label{sec:signatures_nebular}

\subsubsection{other?}
% \label{sec:signatures_}













\section{Intrinsic Rates}

The most direct estimate on the merger rate in the local Universe comes from \ac{GW} observations. We take the most up to date \ac{LIGO} merger rates for \ac{BNS} mergers from \citet{GW170817-GW}, \ac{BBH} mergers from \citet{GW170104}, and the \ac{NSBH} merger rates from \citet{overview_NSMs_GWs_2010}. The \ac{BNS} and \ac{BBH} merger rates have about an order of magnitude uncertainty for the 90\% interval. Because of the lack of direct \ac{GW} observations and the lack of any known \ac{NSBH} system, the \ac{NSBH} 90\% interval spans a few orders of magnitude. These values are given in Table \ref{tab:nearby_rates}. 

These values are the merger rates in the nearby universe. It is generally assumed that compact objects follow the stellar formation rate modulo inspiral times. Therefore, the rate increases out to a redshift of about 1, then decreases until 0 at a time when no mergers occur. We use the form


which has been used in the literature \citep{COB_rate_evo_Schneider_2001, COB_cutler_2009}. This is only a representative parametrization of the evolution of merger rates. It allows for evolution that roughly matches expectations. We do not expect the rate to drop to 0 so sharply, but this is reasonable enough for our other studies. The cumulative intrinsic rate as a function of distance for each of these progenitors is given in Figure \ref{fig:rates_CO}. We see that we go from rare events in the nearby universe up to millions of mergers per year throughout the Universe, which could be observed with Gen 3 detectors.



These rates can be converted into other numbers of interest. Closer events can be far better studied, thus in Table \ref{tab:nearby_rates} we show the closest event in a given time period. The nearby distances are relatively robust given their volumetric nature, e.g. an order of magnitude in rate corresponds to about a factor of two in distances. Therefore, we can expect a \ac{BNS} merger at about 25 Mpc once a decade and \ac{BBH} mergers at about 60 Mpc in the same time period. These events will provide unique information as they can be better studied than more distant events, and the knowledge they provide can be extrapolated to the population.



\section{Assumed Ground-Based \ac{GW} Network Sensitivities and Detection Rates}
\label{sec:GW_detection_rates}

\textcolor{red}{173 Mpc}

The sensitivity of ground-based interferometers is generally quoted by two distance measures: the range and the horizon to canonical (1.4 M$_{\odot}$) \ac{BNS} mergers. This is because we know have observed \ac{NS} around this mass range, and the full distribution should be relatively constrained (e.g. \ac{NS} can only be so small or they would be white dwarfs, and can only be so large or they would become black holes).

\ac{GW} emission is relatively omnidirectional but not isotropic, with the strength stronger along the total angular momentum axis (generally perpendicular to the orbital plane). Similarly, \ac{GW} interferometers are omni directional but not isotropic, with the sensitivity maximized directly above and below the plane of the interferometer arms. The range is radius for a sphere containing equivalent volume to the spacetime volume exposure of the antenna pattern. The horizon is the maximal distance a canonical \ac{BNS} merger can be detected to, which is (for a given interferometer) 2.26 times the range and is for a face-on merger directly overhead (or 180 degrees from) the interferometer.

The range and horizon of a network are somewhat more complicated. The Advanced \ac{LIGO} interferometers are coaligned, so their antenna response patterns are aligned. However, the other interferometers are not coaligned. For example, Virgo has maximal sensitivity to other parts of the sky than \ac{LIGO}. This has the effect of smoothing out the network sensitivity over the sky, significantly increasing the range but not the horizon. The placement of the other interferometers in the network was influenced by approaching a relatively isotropic sensitivity on the sky.

Within a few years we expect to have 5 Gen 2 interferometers active within the same network. There are proposals for Gen 2.5 \textcolor{blue}{interferometers only in the United States}. We do not expect to have 5 Gen 3 interferometers. Therefore, as new interferometers come online we may not expect to maintain the mostly isotropic nature of the design Gen 2 network.

The most sensitive \ac{GW} interferometer achieved a \ac{BNS} range of about 100 Mpc (LIGO-Livingston near the end of the O2 run; \citealt{GW170817-GW}). 


\section{SGRB Rates: Detected and Intrinsic}













astro formation


% \acp{NS} and \acp{BH} are produced when massive stars undergo supernova. Stars between about 8 and 20 $M_{\odot}$ produce \ac{NS} remnants, with heavier stars producing \ac{BH} remnants. The separation between a \ac{NS} or \ac{BH} remnant is set by the maximum mass of a \ac{NS}, M$_{NS}^{Max}$ (see Section \ref{sec:max_NS_mass}). The first known \ac{BNS} system is the Hulse-Taylor Pulsar (PSR 1913+16; \citealt{Hulse_Taylor_pulsar_discovery}), though it wasn't immediately known that the second star in the binary was a \ac{NS}. This pulsar will not merge for some 300 million years, which suggests that \ac{NS} mergers do occur within a Hubble time.


Since this paper is only concerned with \ac{NS} mergers we summarize the standard formation channel for \ac{BNS} and \ac{NSBH} mergers that will merge within a Hubble Time. Such systems begin as a binary system with two high mass stars. As the lifetimes of stars is inversely proportional to the mass of the star, the more massive dies first. By convention, we refer to the more massive star as the primary. The resulting system now contains a compact object (either a \ac{NS} or a \ac{BH}, depending on whether the mass is above or below the maximum mass of a \ac{NS}, M$_{NS}^{Max}$, see Section \ref{sec:max_NS_mass}) and a massive star. At these distances the objects will not merge for an eternity. The resolution has the secondary star expand in the late stages of its life, encompassing the primary compact object; this is the common envelop stage. Here a few things happen: the primary becomes more massive as it devours its friend, the stars move closer together through \textcolor{blue}{dynamical} friction between the outer envelope and the compact object, and the compact object \textcolor{blue}{will unbind parts of its companion's envelop, accelerating the death-knells of the secondary}. If the primary is a \ac{NS}, this accretion may push the primary over M$_{NS}^{Max}$, where it would collapse into a \ac{BH}. Soon the remaining massive star will undergo a supernova explosion and produce a secondary compact object less massive than the primary. If the system remains bound and is sufficiently close then we have a \ac{BNS} or \ac{NSBH} system that can merge within a Hubble Time.

\textcolor{red}{We were pretty sure that at least some \ac{BNS} systems merged within a Hubble time based on the system CITE that will merge in 85 Myr, because a Hubble time plus 85 Myr is basically a Hubble time. However, with the \ac{GW} signal and the associated \ac{EM} transients we confidently detected a \ac{BNS} merger, and thus directly proved they merge in a Hubble time. We will likely need \ac{EM} confirmation of a given signal as having an \ac{NS} progenitor for some time.} However, based on these observations we cannot rule out an equal mass binary, and the spin of the primary was constrained to only $\sim<$0.5 in dimensionless spin units \citep{GW170817_GW_updated_parameters}. \textcolor{red}{The inspiral was consistent with a circular orbit...} \textcolor{red}{The papers on NGC 4993/relation. Levan/Tanvir, LVC, etc}

\textcolor{red}{make this the new subsection?}
There are other channels for the formation of compact object binaries. Dynamical capture is another accepted possible scenario \textcolor{orange}{cite}, but the rates are much more uncertain. Another option for possible merging is dynamic collision where these objects directly hit each other without inspiral. Here we would not see the \ac{GW} inspiral and likely not a \ac{SGRB}, but we may see a burst of \ac{GW} and kilonova-like emission.

Understanding the dominant formation channel for these systems and their merger rates allow us to infer much more about the stellar formation history of galaxies. Population synthesis models are powerful tools to learn more about the universe, but they require observations to calibrate them. \ac{GW} observations of the mergers of these systems provide such a quantity. \textcolor{red}{Stellar population studies are related and tighter constraints on unique systems can provide useful constraints for other studies.}

\textcolor{red}{discuss host galaxy type?}

% \gwid required \ac{EM} observations to classify the progenitors. While with updated parameter estimation and an assumed low-spin prior (based on the observations of galactic \ac{NS}) allowed them to find evidence for a tidal term in the waveform \citep{GW170817_GW_updated_parameters} it may not be absolute proof of a \ac{NS} progenitor alone, and it would only confirm that one of the compact objects was a \ac{NS}. \grbid immediately confirmed that at least one of the progenitors was a \ac{NS} based on the well-found (but previously circumstantial) theory on the origin of \acp{SGRB} (but see Section \ref{sec:unexpected}). The observations of \knid, the bright early behavior, and the inferred ejecta masses all point to a \ac{BNS} merger progenitor over a \ac{NSBH} merger based on kilonova theory and simulations. This shows the power of multimessenger astronomy. 

In the future we require confident classifications of many \ac{GW} triggers. Methods for doing this are discussed in Section \ref{sec:classification}. The standard formation channel will produce some observable signatures: the primary should be both heavier and more rapidly spinning as it is spun-up from accretion during the common envelope stage \textcolor{orange}{180,73 from faber/rasio}. The supernova explosion kick will produce high velocity binary systems, which may result in them being outside, or even unbound, from their host galaxy when they merge after some time. An expected offset distribution can be calculated \textcolor{orange}{cite}, and because of the reasonable match to the observed offsets of \acp{SGRB} to their putative hosts, this was seen as evidence of \ac{NS} mergers as the progenitors of \acp{SGRB}.

\ac{LISA} will detecting millions of galactic binaries (including white dwarfs). \ac{EM} surveys like GAIA, ZTF, and LSST \textcolor{orange}{citations} we will learn far more about stellar populations than from observations of compact object mergers. \ac{LISA} is expected to launch in 2034 and has an outstanding data science problem: how to pull out individual sources when millions of sources are observed through a single data stream. Detections of \ac{NS} mergers over the next decade will inform the \ac{LISA} expectations by providing calibration information (direct measures of the ends of these systems) for population synthesis models. \textcolor{blue}{Indeed most of these models underpredicted the LIGO/Virgo merger rates}. Observing the mergers provides unique insight into the tail of events that merge in a Hubble time. More importantly, by the time \ac{LISA} is taking data we will hopefully have upgraded ground-based \ac{GW} interferometers that can detect these mergers to vast cosmological distances. This provides us insight into the rate evolution of these sources as a function of cosmic time. These complementary observations will provide us with unique insights unavailable to galactic or cosmological observations alone.





\subsubsection{Do Neutron Star-Black Hole Systems exist?}
\label{sec:NSBH_exist}
In Section \ref{sec:overview_formation} we belied an important point: there is no known \ac{NSBH} system. \ac{NSBH} systems are thought to be formed in a similar channel as \ac{BNS} systems, but where the primary object is born, or grows through accretion, massive enough to be a \ac{BH}. These systems may also result from dynamical capture. There is one system that is a candidate for becoming a \ac{NSBH} system in the future \textcolor{orange}{cite}. 

Separate information for \ac{BNS} and \ac{NSBH} systems provide separate calibration points for population synthesis codes (\textcolor{blue}{see e.g. \citealt{population_synthesis_belczynski_2008}}), provide unique insight into the relative abundances of these systems, and thus information on the differences in stellar formation (e.g. the role of metallicities). The unambiguous detection of a \ac{NSBH} merger necessitates a prior \ac{NSBH} progenitor system.

These topics are included here because with respect to our sources of interest they result in the underlying question: what are the differences between \ac{BNS} and \ac{NSBH} mergers? For \acp{SGRB} there are several questions: do \ac{NSBH} mergers cause \acp{SGRB}? If so, what fraction of \acp{SGRB} arise from \ac{BNS} mergers, \ac{NSBH} mergers, or possibly something else? Are \ac{NSBH} \acp{SGRB} more luminous than those from \ac{BNS} mergers (as may be expected due to the steeper gravitational gradient)? For kilonova we have other questions: what \ac{NS} mergers produce what types (red or blue or otherwise) kilonova? What are the relative ejecta masses and velocities? Their distributions? Are \ac{NSBH} kilonova brighter or dimmer than \ac{BNS} mergers? What are the relative lanthanide/actinide productions in each? And a general question: do some \ac{NSBH} (those with higher mass \ac{BH} and lower spins) swallow the \ac{NS} whole? It is expected that \textcolor{blue}{if the tidal disruption radius is smaller than the radius of the innermost stable circular orbit then the \ac{NS} will be swallowed whole, with less massive and faster spinning \ac{BH} more likely to disrupt the \ac{NS}.} With a large enough population we could ask, how do the mass ratio, \ac{BH} mass, and \ac{BH} spin affect the \ac{EM} counterparts (\acp{SGRB}, kilonovae, and others)? We consider this to be a science driver for future observations, but this answer could be uncovered with current capabilities if the rate of \ac{NSBH} mergers are sufficiently high.

To confidently declare a system as arising from the merging of a \ac{NS} and a \ac{BH} we have to have absolute proof for a \ac{NS} and a \ac{BH}. This can, in principle, be uncovered in several ways. The involvement of a \ac{NS} can be inferred from finding evidence for a tidal term in \ac{GW} (with some reasonable assumptions, there is mild evidence for tidal deformation in \gwid \citep{GW170817_GW_updated_NS_EOS} or evidence of a \ac{HMNS} or a \ac{SMNS}, detecting and unambiguously associating a \ac{EM} signal (see Section \ref{sec:associating} for association, or \textcolor{red}{possibly through the detection and association of neutrinos} \textcolor{orange}{cite - could these arise for NSBH mergers or just NS}. The involvement of a \ac{BH} can be inferred by constraining the mass of the primary to be above the maximum mass of a \ac{NS} (see Section \ref{sec:max_NS_mass}), or by matching \ac{EM} observations to theoretical expectations. Details are given in Appendix \ref{sec:classification}. Currently our expectations for the differences between \ac{BNS} and \ac{NSBH} mergers for kilonova are likely easier to differentiate, though there are some possible signals from \acp{SGRB} observations that would be smoking guns (e.g. a quasi-periodic signal showing precession of the orbital plane with respect to the misaligned spin axis of the \ac{BH}). \textcolor{blue}{what about the mass gap paper}. 

This topic benefits from more sensitive \ac{GW} ground-based detectors in both low frequencies (to increase the detection distance and therefore rate) and in high frequencies (to allow direct measurements of the \ac{NS} measurement), better gamma-ray sky coverage and sensitivity, and \textcolor{blue}{improvements to the follow-up searches for red kilonova (\ac{IR} and optical) as we do not expect blue kilonova from these mergers}.

In 400 years of \ac{EM} astronomy no \ac{NSBH} system has been identified. Humanity has identified one system as a candidate for becoming such a system in the future \textcolor{orange}{citation}, but even this is ambiguous. \ac{LISA} will uncover millions of binaries, but \textcolor{cyan}{based on the inferred rates from the current non-detection by \ac{LIGO}/Virgo it appears unlikely that \ac{LISA} will detect a \ac{NSBH} within its observing volume.} We thus consider this an important and unique scientific driver for the future development of the field.


